CSG: A stochastic gradient method for a wide class of optimization problems appearing in a machine learning or data-driven context

A recent article introduced thecontinuous stochastic gradient method (CSG) for the efficient solution of a class of stochastic optimization problems. While the applicability of known stochastic gradient type methods is typically limited to expected risk functions, no such limitation exists for CSG. This advantage stems from the computation of design dependent integration weights, allowing for optimal usage of available information and therefore stronger convergence properties. However, the nature of the formula used for these integration weights essentially limited the practical applicability of this method to problems in which stochasticity enters via a low-dimensional and sufficiently simple probability distribution. In this paper we significantly extend the scope of the CSG method by presenting alternative ways to calculate the integration weights. A full convergence analysis for this new variant of the CSG method is presented and its efficiency is demonstrated in comparison to more classical stochastic gradient methods by means of a number of problem classes relevant to stochastic optimization and machine learning.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Prevent itemized lists from running into the left margin inside theorems and proofs
\usepackage{enumitem}
\setlist[enumerate]{leftmargin=.5in}
\setlist[itemize]{leftmargin=.5in}

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{An Example Article}{D. Doe, P. T. Frank, and J. E. Smith}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{An Example Article\thanks{Submitted to the editors DATE.
\funding{This work was funded by the Fog Research Institute under contract no.~FRI-454.}}}

% Authors: full names plus addresses.
\author{Dianne Doe\thanks{Imagination Corp., Chicago, IL 
  (\email{ddoe@imag.com}, \url{http://www.imag.com/\string~ddoe/}).}
\and Paul T. Frank\thanks{Department of Applied Mathematics, Fictional University, Boise, ID 
  (\email{ptfrank@fictional.edu}, \email{jesmith@fictional.edu}).}
\and Jane E. Smith\footnotemark[3]}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 


==> reference_siam_doi.tex <==
@misc{tan2016barzilaiborwein,
      title={Barzilai-Borwein Step Size for Stochastic Gradient Descent}, 
      author={Conghui Tan and Shiqian Ma and Yu-Hong Dai and Yuqiu Qian},
      year={2016},
      eprint={1605.04131},
      archivePrefix={arXiv},
      primaryClass={math.OC}
}

@book {UniformCone,
    AUTHOR = {Adams, Robert A. and Fournier, John J. F.},
     TITLE = {Sobolev spaces},
    SERIES = {Pure and Applied Mathematics (Amsterdam)},
    VOLUME = {140},
   EDITION = {Second},
 PUBLISHER = {Elsevier/Academic Press, Amsterdam},
      YEAR = {2003},
     PAGES = {xiv+305},
      ISBN = {0-12-044143-8},
   MRCLASS = {46E35 (46-01 46-02 46B70 46Exx)},
  MRNUMBER = {2424078},
}

@article {subgradients,
    AUTHOR = {Alber, Ya. I. and Iusem, A. N. and Solodov, M. V.},
     TITLE = {On the projected subgradient method for nonsmooth convex
              optimization in a {H}ilbert space},
   JOURNAL = {Math. Programming},
  FJOURNAL = {Mathematical Programming},
    VOLUME = {81},
      YEAR = {1998},
    NUMBER = {1, Ser. A},
     PAGES = {23--35},
      ISSN = {0025-5610},
   MRCLASS = {90C25 (49J52 90C48)},
  MRNUMBER = {1617701},
MRREVIEWER = {Lionel Thibault},
       DOI = {10.1007/BF01584842},
       URL = {https://doi.org/10.1007/BF01584842},
}

@book{Schmidt2011,
    author={Schmidt, Klaus D.},
    title={Konvergenz von Folgen von Zufallsvariablen},
    bookTitle={Ma{\ss} und Wahrscheinlichkeit},
    year={2011},
    publisher={Springer Berlin Heidelberg},
    address={Berlin, Heidelberg},
    pages={331--336},
    abstract={Zur Vorbereitung auf die Gesetze der Gro{\ss}en Zahlen, die wir im n{\"a}chsten Kapitel behandeln, vergleichen wir in diesem Kapitel die aus der Ma{\ss}- und Integrationstheorie bekannten drei Arten der Konvergenz f{\"u}r eine Folge von Zufallsvariablen:},
    isbn={978-3-642-21026-6},
    doi={10.1007/978-3-642-21026-6_14},
    url={https://doi.org/10.1007/978-3-642-21026-6_14}
}

@book {Aubin,
    AUTHOR = {Aubin, Jean-Pierre},
     TITLE = {Applied functional analysis},
    SERIES = {Pure and Applied Mathematics (New York)},
   EDITION = {Second},
      NOTE = {With exercises by Bernard Cornet and Jean-Michel Lasry,
              Translated from the French by Carole Labrousse},
 PUBLISHER = {Wiley-Interscience, New York},
      YEAR = {2000},
     PAGES = {xviii+495},
      ISBN = {0-471-17976-0},
   MRCLASS = {46Nxx (47Nxx 49J53)},
  MRNUMBER = {1782330},
MRREVIEWER = {S. D. Chatterji},
}

@BOOK{David2003,
	AUTHOR = {David, Herbert A. AND Nagaraja, H. N.},
	YEAR = {2003},
	TITLE = {Order Statistics - },
	EDITION = {},
	ISBN = {978-0-471-38926-2},
	PUBLISHER = {Wiley},
	ADDRESS = {New York},
}

@book{klenke2013probability,
  AUTHOR = {Klenke, Achim},
     TITLE = {Probability theory},
    SERIES = {Universitext},
      NOTE = {A comprehensive course,
              Translated from the 2006 German original},
 PUBLISHER = {Springer-Verlag London, Ltd., London},
      YEAR = {2008},
     PAGES = {xii+616},
      ISBN = {978-1-84800-047-6},
   MRCLASS = {60-01 (28-01 60B10 60F05 60F15 60G42 60J10)},
  MRNUMBER = {2372119},
MRREVIEWER = {Sophie Lemaire},
}


@article{Bottou2016,
  AUTHOR = {Bottou, L\'{e}on and Curtis, Frank E. and Nocedal, Jorge},
     TITLE = {Optimization methods for large-scale machine learning},
   JOURNAL = {SIAM Rev.},
  FJOURNAL = {SIAM Review},
    VOLUME = {60},
      YEAR = {2018},
    NUMBER = {2},
     PAGES = {223--311},
      ISSN = {0036-1445},
   MRCLASS = {65K05 (68Q25 68T05 90C06 90C30 90C90)},
  MRNUMBER = {3797719},
MRREVIEWER = {Boualem Alleche},
}

@article {Monro1951,
    AUTHOR = {Robbins, Herbert and Monro, Sutton},
     TITLE = {A stochastic approximation method},
   JOURNAL = {Ann. Math. Statistics},
  FJOURNAL = {Annals of Mathematical Statistics},
    VOLUME = {22},
      YEAR = {1951},
     PAGES = {400--407},
      ISSN = {0003-4851},
   MRCLASS = {62.0X},
  MRNUMBER = {42668},
MRREVIEWER = {R. P. Peterson},
       DOI = {10.1214/aoms/1177729586},
       URL = {https://doi.org/10.1214/aoms/1177729586},
}


@BOOK{Knopp1922,
	AUTHOR = {Knopp, Conrad},
	YEAR = {1922},
	TITLE = {Theorie und Anwendung der unendlichen Reihen, von Dr. Konrad Knopp, ... - },
	EDITION = {},
	ISBN = {},
	PUBLISHER = {J. Springer},
	ADDRESS = {Berlin},
}

@article {LeRoux2017,
    AUTHOR = {Schmidt, Mark and Le Roux, Nicolas and Bach, Francis},
     TITLE = {Minimizing finite sums with the stochastic average gradient},
   JOURNAL = {Math. Program.},
  FJOURNAL = {Mathematical Programming},
    VOLUME = {162},
      YEAR = {2017},
    NUMBER = {1-2, Ser. A},
     PAGES = {83--112},
      ISSN = {0025-5610},
   MRCLASS = {90C25 (62L20 65K05 68Q25 90C06 90C15)},
  MRNUMBER = {3612933},
       DOI = {10.1007/s10107-016-1030-6},
       URL = {https://doi.org/10.1007/s10107-016-1030-6},
}



@article{Zhang2017,
title = "Stochastic sampling for deterministic structural topology optimization with many load cases: Density-based and ground structure approaches",
journal = "Computer Methods in Applied Mechanics and Engineering",
volume = "325",
pages = "463 - 487",
year = "2017",
author = "Xiaojia Shelly Zhang and Eric de Sturler and Glaucio H. Paulino"
}

@Book{werner2005,
 author = {Werner, D},
 title = {Funktionalanalysis},
 publisher = {Springer},
 year = {2005},
 address = {Berlin},
 isbn = {9783540267492}
 }
 
 @Article{Calamai1987,
author="Calamai, Paul H.
and Mor{\'e}, Jorge J.",
title="Projected gradient methods for linearly constrained problems",
journal="Mathematical Programming",
year="1987",
month="Sep",
day="01",
volume="39",
number="1",
pages="93--116",
issn="1436-4646",
doi="10.1007/BF02592073",
url="https://doi.org/10.1007/BF02592073"
}

@Book{nocedal2006,
 author = {Nocedal, Jorge},
 title = {Numerical optimization},
 publisher = {Springer},
 year = {2006},
 address = {New York},
 isbn = {978-0-387-40065-5}
 }
 
 @BOOK{Bertsekas2016,
	AUTHOR = {Bertsekas, Dimitri P.},
	YEAR = {2016},
	TITLE = {Nonlinear Programming - },
	EDITION = {2},
	ISBN = {978-1-886-52905-2},
	PUBLISHER = {Athena Scientific},
	ADDRESS = {Belmont, Massachusetts},
}

@BOOK{Zarantonello1971,
	AUTHOR = {Zarantonello, Eduardo H.},
	YEAR = {1971},
	TITLE = {Projections on Convex Sets in Hilbert Space and Spectral Theory - },
	EDITION = {},
	ISBN = {},
	PUBLISHER = {University of Wisconsin},
	ADDRESS = {},
}

@Article{Bendsoe1989,
author="Bends{\o}e, M. P.",
title="Optimal shape design as a material distribution problem",
journal="Structural optimization",
year="1989",
month="Dec",
day="01",
volume="1",
number="4",
pages="193--202",
issn="1615-1488",
}

@Article{Sigmund1998,
author="Sigmund, O.
and Petersson, J.",
title="Numerical instabilities in topology optimization: A survey on procedures dealing with checkerboards, mesh-dependencies and local minima",
journal="Structural optimization",
year="1998",
month="Aug",
day="01",
volume="16",
number="1",
pages="68--75",
issn="1615-1488",
doi="10.1007/BF01214002",
url="https://doi.org/10.1007/BF01214002"
}

@article{stingl2018,
author = {Semmler, J. and Pflug, L. and Stingl, M.},
title = {Material Optimization in Transverse Electromagnetic Scattering Applications},
journal = {SIAM Journal on Scientific Computing},
volume = {40},
number = {1},
pages = {B85-B109},
year = {2018}
}

@book{rudin1964principles,
  title={Principles of mathematical analysis},
  author={Rudin, Walter and others},
  volume={3},
  year={1964},
  publisher={McGraw-hill New York}
}

@inproceedings{bottou2004,
  title={Large scale online learning},
  author={Bottou, L{\'e}on and Cun, Yann L},
  booktitle={Advances in neural information processing systems},
  pages={217--224},
  year={2004}
}
@article{diaz1992,
  title={Shape optimization of structures for multiple loading conditions using a homogenization method},
  author={Diaz, AR and Bends{\o}e, MPe},
  journal={Structural optimization},
  volume={4},
  number={1},
  pages={17--22},
  year={1992},
  publisher={Springer}
}
@article{gersborg2006,
  title={Topology optimization of heat conduction problems using the finite volume method},
  author={Gersborg-Hansen, Allan and Bends{\o}e, Martin P and Sigmund, Ole},
  journal={Structural and multidisciplinary optimization},
  volume={31},
  number={4},
  pages={251--259},
  year={2006},
  publisher={Springer}
}
@article{de2019,
  title={Topology Optimization under Uncertainty using a Stochastic Gradient-based Approach},
  author={De, Subhayan and Hampton, Jerrad and Maute, Kurt and Doostan, Alireza},
  journal={arXiv preprint arXiv:1902.04562},
  year={2019}
}
@article{conti2009,
  title={Shape optimization under uncertainty—a stochastic programming perspective},
  author={Conti, Sergio and Held, Harald and Pach, Martin and Rumpf, Martin and Schultz, R{\"u}diger},
  journal={SIAM Journal on Optimization},
  volume={19},
  number={4},
  pages={1610--1632},
  year={2009},
  publisher={SIAM}
}
@article{evgrafov2003,
  title={Stochastic structural topology optimization: discretization and penalty function approach},
  author={Evgrafov, Anton and Patriksson, Michael},
  journal={Structural and Multidisciplinary Optimization},
  volume={25},
  number={3},
  pages={174--188},
  year={2003},
  publisher={Springer}
}
@article{alvarez2005,
  title={Minimization of the expected compliance as an alternative approach to multiload truss optimization},
  author={Alvarez, Felipe and Carrasco, Miguel},
  journal={Structural and Multidisciplinary optimization},
  volume={29},
  number={6},
  pages={470--476},
  year={2005},
  publisher={Springer}
}
@article{guo2015,
  title={Multi-scale robust design and optimization considering load uncertainties},
  author={Guo, Xu and Zhao, Xiaofang and Zhang, Weisheng and Yan, Jun and Sun, Guomin},
  journal={Computer Methods in Applied Mechanics and Engineering},
  volume={283},
  pages={994--1009},
  year={2015},
  publisher={Elsevier}
}
@article{guest2008,
  title={Structural optimization under uncertain loads and nodal locations},
  author={Guest, James K and Igusa, Takeru},
  journal={Computer Methods in Applied Mechanics and Engineering},
  volume={198},
  number={1},
  pages={116--124},
  year={2008},
  publisher={Elsevier}
}
@article{christiansen2001,
  title={Stochastic bilevel programming in structural optimization},
  author={Christiansen, Snorre and Patriksson, Michael and Wynter, Laura},
  journal={Structural and multidisciplinary optimization},
  volume={21},
  number={5},
  pages={361--371},
  year={2001},
  publisher={Springer}
}

@Article{Sigmund2013,
author="Sigmund, Ole
and Maute, Kurt",
title="Topology optimization approaches",
journal="Structural and Multidisciplinary Optimization",
year="2013",
month="Dec",
day="01",
volume="48",
number="6",
pages="1031--1055"
}

@Article{Dilgen2019,
author="Dilgen, Cetin B.
and Dilgen, Sumer B.
and Aage, Niels
and Jensen, Jakob S.",
title="Topology optimization of acoustic mechanical interaction problems: a comparative review",
journal="Structural and Multidisciplinary Optimization",
year="2019",
month="Aug",
day="01",
volume="60",
number="2",
pages="779--801"
}

@article{doi:10.1002/lpor.201000014,
author = {Jensen, J.S. and Sigmund, O.},
title = {Topology optimization for nano-photonics},
journal = {Laser \& Photonics Reviews},
volume = {5},
number = {2},
pages = {308-321},
keywords = {Topology optimization, nano-photonics, material distribution, sensitivity analysis, math-programming.},
year = {2011}
}

@article{MAUTE2003813,
title = "Reliability-based design of MEMS mechanisms by topology optimization",
journal = "Computers \& Structures",
volume = "81",
number = "8",
pages = "813 - 824",
year = "2003",
note = "K.J Bathe 60th Anniversary Issue",
author = "Kurt Maute and Dan M. Frangopol"
}

@Article{ Svanberg:02,
    title = "A class of globally convergent optimization methods based on conservative convex separable approximations",
    journal = "SIAM Journal on Optimization",
    volume = "12",
    number = "2",
    year = "2002",
    pages = "555--573",
    author = "K. Svanberg"
}


@article{doi:10.1137/130922756,
author = {Roosta-Khorasani, F. and van den Doel, K. and Ascher, U.},
title = {Stochastic Algorithms for Inverse Problems Involving PDEs and many Measurements},
journal = {SIAM Journal on Scientific Computing},
volume = {36},
number = {5},
pages = {S3-S22},
year = {2014}
}


@article{doi:10.1137/11081126X,
author = {Haber, E. and Chung, M. and Herrmann, F.},
title = {An Effective Method for Parameter Estimation with PDE Constraints with Multiple Right-Hand Sides},
journal = {SIAM Journal on Optimization},
volume = {22},
number = {3},
pages = {739-757},
year = {2012}
}

@incollection{Semmler2015,
  year = {2015},
  publisher = {Springer International Publishing},
  pages = {251--269},
  author = {Johannes Semmler and Lukas Pflug and Michael Stingl and G\"{u}nter Leugering},
  title = {Shape Optimization in Electromagnetic Applications},
  booktitle = {New Trends in Shape Optimization}
}

@book{jahn2007introduction,
  title={Introduction to the theory of nonlinear optimization},
  author={Jahn, Johannes},
  year={2007},
  publisher={Springer Science \& Business Media}
}
@incollection{Tan2016,
title = {Barzilai-Borwein Step Size for Stochastic Gradient Descent},
author = {Tan, Conghui and Ma, Shiqian and Dai, Yu-Hong and Qian, Yuqiu},
booktitle = {Advances in Neural Information Processing Systems 29},
editor = {D. D. Lee and M. Sugiyama and U. V. Luxburg and I. Guyon and R. Garnett},
pages = {685--693},
year = {2016},
publisher = {Curran Associates, Inc.},
}

@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}
@article{dudley1969speed,
  title={The speed of mean Glivenko-Cantelli convergence},
  author={Dudley, Richard Mansfield},
  journal={The Annals of Mathematical Statistics},
  volume={40},
  number={1},
  pages={40--50},
  year={1969},
  publisher={JSTOR}
}
@incollection{fortune1995voronoi,
  title={Voronoi diagrams and Delaunay triangulations},
  author={Fortune, Steven},
  booktitle={Computing in Euclidean geometry},
  pages={225--265},
  year={1995},
  publisher={World Scientific}
}
@book{burgisser2013condition,
  title={Condition: The geometry of numerical algorithms},
  author={B{\"u}rgisser, Peter and Cucker, Felipe},
  volume={349},
  year={2013},
  publisher={Springer Science \& Business Media}
}
@inproceedings{shewchuk1996triangle,
  title={Triangle: Engineering a 2D quality mesh generator and Delaunay triangulator},
  author={Shewchuk, Jonathan Richard},
  booktitle={Workshop on Applied Computational Geometry},
  pages={203--222},
  year={1996},
  organization={Springer}
}
@inproceedings{barron1992neural,
  title={Neural net approximation},
  author={Barron, Andrew R},
  booktitle={Proc. 7th Yale Workshop on Adaptive and Learning Systems},
  volume={1},
  pages={69--72},
  year={1992}
}

@inproceedings{lecun1988theoretical,
  title={A theoretical framework for back-propagation},
  author={LeCun, Yann and Touresky, D and Hinton, G and Sejnowski, T},
  booktitle={Proceedings of the 1988 connectionist models summer school},
  volume={1},
  pages={21--28},
  year={1988},
  organization={CMU, Pittsburgh, Pa: Morgan Kaufmann}
}

@article{hardt2015train,
  title={Train faster, generalize better: Stability of stochastic gradient descent},
  author={Hardt, Moritz and Recht, Benjamin and Singer, Yoram},
  journal={arXiv preprint arXiv:1509.01240},
  year={2015}
}
@Article{Fournier2015,
author="Fournier, Nicolas
and Guillin, Arnaud",
title="On the rate of convergence in Wasserstein distance of the empirical measure",
journal="Probability Theory and Related Fields",
year="2015",
month="Aug",
day="01",
volume="162",
number="3",
pages="707--738"
}

@article{Feinberg2014,
  title={Fatou's lemma for weakly converging probabilities},
  author={Feinberg, Eugene A and Kasyanov, Pavlo O and Zadoianchuk, Nina V},
  journal={Theory of Probability \& Its Applications},
  volume={58},
  number={4},
  pages={683--689},
  year={2014},
  publisher={SIAM}
}
@article{gibbs2002choosing,
  title={On choosing and bounding probability metrics},
  author={Gibbs, Alison L and Su, Francis Edward},
  journal={International statistical review},
  volume={70},
  number={3},
  pages={419--435},
  year={2002},
  publisher={Wiley Online Library}
}

@book{billingsley2013convergence,
  AUTHOR = {Billingsley, Patrick},
     TITLE = {Convergence of probability measures},
    SERIES = {Wiley Series in Probability and Statistics: Probability and
              Statistics},
   EDITION = {Second},
      NOTE = {A Wiley-Interscience Publication},
 PUBLISHER = {John Wiley \& Sons, Inc., New York},
      YEAR = {1999},
     PAGES = {x+277},
      ISBN = {0-471-19745-9},
   MRCLASS = {60B10 (28A33 60F17)},
  MRNUMBER = {1700749},
}

@book{folland2009guide,
  AUTHOR = {Folland, Gerald B.},
     TITLE = {A guide to advanced real analysis},
    SERIES = {The Dolciani Mathematical Expositions},
    VOLUME = {37},
      NOTE = {MAA Guides, 2},
 PUBLISHER = {Mathematical Association of America, Washington, DC},
      YEAR = {2009},
     PAGES = {x+107},
      ISBN = {978-0-88385-343-6},
   MRCLASS = {46-01 (26-01 26Axx 28-01)},
  MRNUMBER = {2528112},
MRREVIEWER = {Lubo\v{s} Pick},
}

@article{pflug_CSG,
    AUTHOR = {Pflug, Lukas and Bernhardt, Niklas and Grieshammer, Max and
              Stingl, Michael},
     TITLE = {C{SG}: a new stochastic gradient method for the efficient
              solution of structural optimization problems with infinitely
              many states},
   JOURNAL = {Struct. Multidiscip. Optim.},
  FJOURNAL = {Structural and Multidisciplinary Optimization},
    VOLUME = {61},
      YEAR = {2020},
    NUMBER = {6},
     PAGES = {2595--2611},
      ISSN = {1615-147X},
   MRCLASS = {90C34 (74P10 90C15 90C48 90C52)},
  MRNUMBER = {4119066},
MRREVIEWER = {Shih-Kang Chao},
}

@article {SCGDPaper,
    AUTHOR = {Wang, Mengdi and Fang, Ethan X. and Liu, Han},
     TITLE = {Stochastic compositional gradient descent: algorithms for
              minimizing compositions of expected-value functions},
   JOURNAL = {Math. Program.},
  FJOURNAL = {Mathematical Programming},
    VOLUME = {161},
      YEAR = {2017},
    NUMBER = {1-2, Ser. A},
     PAGES = {419--449},
      ISSN = {0025-5610},
   MRCLASS = {90C15 (68W27 90C06 90C25)},
  MRNUMBER = {3592784},
MRREVIEWER = {Vlasta Ka\v{n}kov\'{a}},
DOI = {10.1007/s10107-016-1017-3},
URL = {https://doi.org/10.1007/s10107-016-1017-3},
}

@article {EmpiricalDistrPaper,
    AUTHOR = {Varadarajan, V. S.},
     TITLE = {On the convergence of sample probability distributions},
   JOURNAL = {Sankhy\={a}},
  FJOURNAL = {Sankhy\={a}. The Indian Journal of Statistics.},
    VOLUME = {19},
      YEAR = {1958},
     PAGES = {23--26},
      ISSN = {0036-4452},
   MRCLASS = {60.00},
  MRNUMBER = {94839},
MRREVIEWER = {M. Lo\`eve},
}

@article {InexProxMeth,
    AUTHOR = {Wang, Xiao and Zhang, Hongchao},
     TITLE = {Inexact proximal stochastic second-order methods for nonconvex
              composite optimization},
   JOURNAL = {Optim. Methods Softw.},
  FJOURNAL = {Optimization Methods \& Software},
    VOLUME = {35},
      YEAR = {2020},
    NUMBER = {4},
     PAGES = {808--835},
      ISSN = {1055-6788},
   MRCLASS = {65K05 (90C26)},
  MRNUMBER = {4121439},
MRREVIEWER = {Warren L. Hare},
       DOI = {10.1080/10556788.2020.1713128},
       URL = {https://doi.org/10.1080/10556788.2020.1713128},
}

@article {LevelSetMeth,
    AUTHOR = {Lin, Qihang and Nadarajah, Selvaprabu and Soheili, Negar and
              Yang, Tianbao},
     TITLE = {A data efficient and feasible level set method for stochastic
              convex optimization with expectation constraints},
   JOURNAL = {J. Mach. Learn. Res.},
  FJOURNAL = {Journal of Machine Learning Research (JMLR)},
    VOLUME = {21},
      YEAR = {2020},
     PAGES = {Paper No. 143, 45},
      ISSN = {1532-4435},
   MRCLASS = {90C15 (62H30 90C25)},
  MRNUMBER = {4138127},
MRREVIEWER = {Wim van Ackooij},
}

@article {PrimDualMeth,
    AUTHOR = {Zhu, Ya-Nan and Zhang, Xiaoqun},
     TITLE = {Stochastic primal dual fixed point method for composite
              optimization},
   JOURNAL = {J. Sci. Comput.},
  FJOURNAL = {Journal of Scientific Computing},
    VOLUME = {84},
      YEAR = {2020},
    NUMBER = {1},
     PAGES = {Paper No. 16, 25},
      ISSN = {0885-7474},
   MRCLASS = {60-08 (62J07 90C15 90C25)},
  MRNUMBER = {4121187},
       DOI = {10.1007/s10915-020-01265-2},
       URL = {https://doi.org/10.1007/s10915-020-01265-2},
}

@article {SARAH,
    AUTHOR = {Nguyen, Lam M. and Scheinberg, Katya and Tak\'{a}\v{c}, Martin},
     TITLE = {Inexact {SARAH} algorithm for stochastic optimization},
   JOURNAL = {Optim. Methods Softw.},
  FJOURNAL = {Optimization Methods \& Software},
    VOLUME = {36},
      YEAR = {2021},
    NUMBER = {1},
     PAGES = {237--258},
      ISSN = {1055-6788},
   MRCLASS = {90C15 (90C25 90C30)},
  MRNUMBER = {4200431},
       DOI = {10.1080/10556788.2020.1818081},
       URL = {https://doi.org/10.1080/10556788.2020.1818081},
}

@article {TRMeth,
    AUTHOR = {Curtis, Frank E. and Scheinberg, Katya and Shi, Rui},
     TITLE = {A stochastic trust region algorithm based on careful step
              normalization},
   JOURNAL = {INFORMS J. Optim.},
  FJOURNAL = {INFORMS Journal on Optimization},
    VOLUME = {1},
      YEAR = {2019},
    NUMBER = {3},
     PAGES = {200--220},
      ISSN = {2575-1484},
   MRCLASS = {90C15 (62J12 62L20 90C55)},
  MRNUMBER = {4154120},
MRREVIEWER = {I. M. Stancu-Minasian},
       DOI = {10.1287/ijoo.2018.0010},
       URL = {https://doi.org/10.1287/ijoo.2018.0010},
}

@article {Patel2016,
    AUTHOR = {Patel, Vivak},
     TITLE = {Kalman-based stochastic gradient method with stop condition
              and insensitivity to conditioning},
   JOURNAL = {SIAM J. Optim.},
  FJOURNAL = {SIAM Journal on Optimization},
    VOLUME = {26},
      YEAR = {2016},
    NUMBER = {4},
     PAGES = {2620--2648},
      ISSN = {1052-6234},
   MRCLASS = {62L12 (62J05 68Q32 90C53 93E35)},
  MRNUMBER = {3576578},
       DOI = {10.1137/15M1048239},
       URL = {https://doi.org/10.1137/15M1048239},
}

@article {Paquette2020,
    AUTHOR = {Paquette, Courtney and Scheinberg, Katya},
     TITLE = {A stochastic line search method with expected complexity
              analysis},
   JOURNAL = {SIAM J. Optim.},
  FJOURNAL = {SIAM Journal on Optimization},
    VOLUME = {30},
      YEAR = {2020},
    NUMBER = {1},
     PAGES = {349--376},
      ISSN = {1052-6234},
   MRCLASS = {90C30 (90C15)},
  MRNUMBER = {4060460},
       DOI = {10.1137/18M1216250},
       URL = {https://doi.org/10.1137/18M1216250},
}

@article{NNMeaningful,
author = {Beyer, Kevin and Goldstein, Jonathan and Ramakrishnan, Raghu and Shaft, Uri},
year = {1997},
month = {12},
pages = {},
title = {When Is "Nearest Neighbor" Meaningful?},
volume = {1540},
journal = {ICDT 1999. LNCS}
}

@article {MonteCarloHighDim,
    AUTHOR = {Yakowitz, S. and Krimmel, J. E. and Szidarovszky, F.},
     TITLE = {Weighted {M}onte {C}arlo integration},
   JOURNAL = {SIAM J. Numer. Anal.},
  FJOURNAL = {SIAM Journal on Numerical Analysis},
    VOLUME = {15},
      YEAR = {1978},
    NUMBER = {6},
     PAGES = {1289--1300},
      ISSN = {0036-1429},
   MRCLASS = {65C05},
  MRNUMBER = {512700},
MRREVIEWER = {Istv\'{a}n D\'{e}ak},
       DOI = {10.1137/0715088},
       URL = {https://doi.org/10.1137/0715088},
}



